Boron depletion in Galactic early B-type stars reveals two different main sequence star populations

The evolution and fate of massive stars are thought to be affected by rotationally induced internal mixing. The surface boron abundance is a sensitive tracer of this in early B-type main sequence stars. We test current stellar evolution models of massive main sequence stars which include rotational mixing through a systematic study of their predicted surface boron depletion. We construct a dense grid of rotating single star models using MESA, for which we employ a new nuclear network which follows all the stable isotopes up to silicon, including lithium, beryllium, boron, as well as the radioactive isotope aluminium-26. We also compile the measured physical parameters of the 90 Galactic early B-type stars with boron abundance information. We then compare each observed stars with our models through a Bayesian analysis, which yields the mixing efficiency parameter with which the star is reproduced the best, and the probability that it is represented by the stellar models. We find that about two-thirds of the sample stars are well represented by the stellar models, with the best agreement achieved for a rotational mixing efficiency of ~50% compared to the widely adopted value. The remaining one third of the stars, of which many are strongly boron depleted slow rotators, are largely incompatible with our models, for any rotational mixing efficiency. We investigate the observational incidence of binary companions and surface magnetic fields, and discuss their evolutionary implications. Our results confirm the concept of rotational mixing in radiative stellar envelopes. On the other hand, we find that a different boron depletion mechanism, and likely a different formation path, is required to explain about one-third of the sample stars. The large spread in the surface boron abundances of these stars may hold a clue to understanding their origin.

==> old_tab_field.tex <==
\begin{table*}[]
\caption{List of our sample of stars that do not belong to NGC\,3293.}
\label{tab_field}
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccccccccccc}
\hline \hline
No & HD number & \begin{tabular}[c]{@{}c@{}}Spectral\\ Type\end{tabular} & $V$ & $B-V$ & \begin{tabular}[c]{@{}c@{}}dist.\\ {[}pc{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}BC\\ {[}mag{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$E(B-V)$\\ {[}mag{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$Mv$\\ {[}mag{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\logL$\\ {[}$\Lsun${}{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$R$\\ {[}$\Rsun${}{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$M_\mathrm{sp}$\\ {[}$\Msun${}{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$M_\mathrm{sp,c}$\\ {[}$\Msun${}{]}\end{tabular} \\ \hline
1 & HD 44743 & B1II-III & 1.98 & -0.24 &  & -2.357 & 0.01 & -3.95 & 4.418 ± 0.056 & 9.4 ± 0.53 & 10.86 ± 4.17 & 10.88 ± 4.17 \\
2 & HD 37023 & B1.5Vp & 6.7 & 0.09 & 500 & -3.071 & 0.385 & -3.37 & 4.472 ± 0.073 & 5.42 ± 0.38 & 55.52 ± 15.34 & 55.61 ± 15.34 \\
3 & HD 34816 & B0.5V & 4.29 & -0.235 & 269.69 & -2.931 & 0.039 & -3.21 & 4.354 ± 0.07 & 5.45 ± 0.39 & 22.35 ± 6.23 & 22.38 ± 6.23 \\
4 & HD 142669 & B2IV-V & 3.87 & -0.199 & 136.58 & -2.065 & 0.018 & -1.99 & 3.518 ± 0.064 & 4.4 ± 0.24 & 9.56 ± 2.44 & 9.8 ± 2.45 \\
5 & HD 63578 & B2III & 5.22 & -0.151 & 458.86 & -2.442 & 0.082 & -3.34 & 4.21 ± 0.077 & 7.15 ± 0.55 & 41.18 ± 11.69 & 41.44 ± 11.71 \\
6 & HD 112092 & B2IV-V & 4.03 & -0.18 & 103.88 & -2.018 & 0.026 & -1.53 & 3.316 ± 0.069 & 3.63 ± 0.2 & 9.8 ± 2.46 & 9.84 ± 2.46 \\
7 & HD 212978 & B2V & 6.16 & -0.136 & 496.65 & -1.94 & 0.067 & -2.53 & 3.686 ± 0.075 & 5.89 ± 0.35 & 10.65 ± 2.83 & 11.08 ± 2.85 \\
8 & HD 36351 & B3II/III & 5.46 & -0.176 &  & -2.181 & 0.042 & -2.24 & 3.663 ± 0.071 & 4.72 ± 0.3 & 12.11 ± 3.2 & 12.16 ± 3.21 \\
9 & HD 160762 & B3IV & 3.82 & -0.179 & 131.99 & -1.613 & 0.014 & -2.15 & 3.402 ± 0.074 & 5.5 ± 0.33 & 7.2 ± 1.88 & 7.2 ± 1.88 \\
11 & HD 35039 & B2IV & 4.72 & -0.168 & 349.81 & -1.894 & 0.039 & -3.12 & 3.903 ± 0.062 & 7.79 ± 0.55 & 8.19 ± 1.78 & 8.2 ± 1.78 \\
12 & HD 35299 & B2III & 5.69 & -0.208 & 360.59 & -2.345 & 0.024 & -2.17 & 3.704 ± 0.063 & 4.31 ± 0.25 & 11.08 ± 2.87 & 11.08 ± 2.87 \\
13 & BD+56 576 & B1.5I & 9.4 & 0.28 & 2530.36 & -2.213 & 0.506 & -4.01 & 4.385 ± 0.074 & 10.33 ± 0.76 & 14.34 ± 4.09 & 14.38 ± 4.09 \\
15 & HD 121790 & B2IV-V & 3.87 & -0.208 & 114.61 & -2.126 & 0.015 & -1.76 & 3.451 ± 0.057 & 3.87 ± 0.18 & 7.95 ± 2 & 8.24 ± 2 \\
16 & HD 36430 & B3V & 6.23 & -0.178 & 397.25 & -1.91 & 0.021 & -1.83 & 3.392 ± 0.071 & 4.31 ± 0.24 & 16 ± 4.13 & 16.02 ± 4.13 \\
17 & HD 64722 & B2IV & 5.7 & -0.151 & 415.3 & -2.462 & 0.087 & -2.66 & 3.945 ± 0.062 & 5.11 ± 0.31 & 11.09 ± 2.93 & 11.51 ± 2.94 \\
18 & HD 36959 & B1V & 5.67 & -0.228 & 358.18 & -2.589 & 0.021 & -2.17 & 3.8 ± 0.047 & 3.9 ± 0.21 & 10 ± 1.98 & 10 ± 1.98 \\
19 & HD 37744 & B2IV & 6.22 & -0.194 & 396.84 & -2.393 & 0.04 & -1.9 & 3.613 ± 0.047 & 3.72 ± 0.19 & 6.52 ± 1.68 & 6.54 ± 1.68 \\
21 & HD 37017 & B2/3V & 6.57 & -0.142 & 359.26 & -1.821 & 0.048 & -1.36 & 3.169 ± 0.078 & 3.58 ± 0.21 & 7.61 ± 1.95 & 7.98 ± 1.96 \\
22 & HD 122980 & B2V & 4.36 & -0.198 & 128.97 & -2.056 & 0.017 & -1.63 & 3.371 ± 0.044 & 3.75 ± 0.18 & 8.58 ± 1.28 & 8.59 ± 1.28 \\
23 & HD 37209 & B2IV & 5.71 & -0.212 & 387.94 & -2.397 & 0.025 & -2.31 & 3.779 ± 0.062 & 4.49 ± 0.27 & 10.22 ± 2.66 & 10.28 ± 2.66 \\
24 & HD 111123 & B1IV & 1.25 & -0.238 &  & -2.673 & 0.022 & -3.48 & 4.358 ± 0.088 & 6.71 ± 0.66 & 8.24 ± 4.54 & 8.32 ± 4.54 \\
25 & HD 36629 & B2V & 7.65 & -0.006 & 429 & -2.226 & 0.21 & -1.22 & 3.274 ± 0.07 & 2.92 ± 0.17 & 7.16 ± 1.84 & 7.16 ± 1.84 \\
26 & HD 37020 & B0V & 6.73 & 0.02 & 500 & -2.955 & 0.294 & -3.03 & 4.288 ± 0.081 & 4.96 ± 0.46 & 18.38 ± 4.9 & 18.43 ± 4.9 \\
28 & HD 37356 & B3V & 6.16 & -0.029 & 455.12 & -2.225 & 0.191 & -2.86 & 3.93 ± 0.076 & 6.19 ± 0.42 & 19.41 ± 5.24 & 19.43 ± 5.24 \\
29 & HD 41753 & B3IV & 4.42 & -0.164 & 147.81 & -1.554 & 0.018 & -1.97 & 3.308 ± 0.08 & 5.18 ± 0.34 & 8.82 ± 2.38 & 8.89 ± 2.39 \\
30 & HD 109668 & B2IV & 2.69 & -0.176 & 116.03 & -2.118 & 0.039 & -2.76 & 3.848 ± 0.106 & 6.18 ± 0.69 & 16.59 ± 5.43 & 17.04 ± 5.46 \\
31 & HD 29248 & B2III & 3.93 & -0.21 & 211.61 & -2.185 & 0.019 & -2.72 & 3.86 ± 0.056 & 5.88 ± 0.37 & 9.05 ± 1.58 & 9.07 ± 1.58 \\
32 & HD 38622 & B2IV-V & 5.28 & -0.156 & 289.03 & -1.61 & 0.031 & -2.12 & 3.389 ± 0.081 & 5.43 ± 0.34 & 4.31 ± 1.14 & 4.37 ± 1.14 \\
33 & HD 120324 & B2Vnpe & 3.47 & -0.17 & 118.54 & -2.225 & 0.056 & -2.38 & 3.739 ± 0.087 & 4.92 ± 0.45 & 5.15 ± 1.55 & 5.8 ± 1.59 \\
34 & HD 202347 & B1V & 7.52 & -0.112 & 776.4 & -2.321 & 0.115 & -2.29 & 3.739 ± 0.069 & 4.58 ± 0.28 & 10.64 ± 2.8 & 10.97 ± 2.81 \\
35 & HD 64740 & B2V & 4.63 & -0.228 & 214.18 & -2.271 & 0.01 & -2.35 & 3.744 ± 0.056 & 4.8 ± 0.25 & 10.88 ± 2.77 & 11.31 ± 2.78 \\
36 & HD 68243 & B2III & 4.173 & -0.178 & 383.85 & -2.407 & 0.058 & -3.92 & 4.429 ± 0.071 & 9.33 ± 0.67 & 27.29 ± 7.58 & 27.71 ± 7.6 \\
37 & HD 45546 & B2V & 5.06 & -0.175 & 306.21 & -1.876 & 0.03 & -1.98 & 3.44 ± 0.09 & 4.67 ± 0.4 & 4.73 ± 1.39 & 4.82 ± 1.4 \\
38 & HD 24131 & B1V & 5.78 & -0.036 & 365.22 & -2.62 & 0.208 & -2.68 & 4.015 ± 0.063 & 4.88 ± 0.29 & 20.62 ± 5.48 & 20.76 ± 5.48 \\
40 & HD 886 & B2IV & 2.83 & -0.19 &  & -2.183 & 0.032 & -3.06 & 3.994 ± 0.082 & 6.89 ± 0.56 & 15.96 ± 4.6 & 15.96 ± 4.6 \\
41 & HD 143018 & B1V+B2:V: & 2.89 & -0.18 &  & -2.708 & 0.073 & -2.41 & 3.944 ± 0.086 & 4.16 ± 0.37 & 10.34 ± 3.09 & 10.59 ± 3.1 \\
42 & HD 216916 & B2IV & 5.6 & -0.149 & 446.69 & -2.287 & 0.078 & -2.89 & 3.967 ± 0.068 & 6.1 ± 0.38 & 12.48 ± 3.28 & 12.48 ± 3.28 \\
43 & HD 121743 & B2IV & 3.83 & -0.224 & 117.49 & -2.146 & 0.009 & -1.94 & 3.532 ± 0.062 & 4.18 ± 0.25 & 7.89 ± 2.07 & 7.99 ± 2.07 \\
44 & HD 35337 & B2IV & 5.25 & -0.219 & 370.25 & -2.355 & 0.018 & -2.65 & 3.897 ± 0.061 & 5.35 ± 0.31 & 17.06 ± 4.51 & 17.07 ± 4.51 \\
48 & HD 180163 & B2.5IV & 4.43 & -0.15 & 262.98 & -1.47 & 0.031 & -3.35 & 3.824 ± 0.082 & 10.03 ± 0.72 & 7.06 ± 1.93 & 7.13 ± 1.94 \\
49 & HD 22951 & B0.5V & 4.97 & -0.048 & 329.92 & -2.752 & 0.207 & -3.52 & 4.404 ± 0.07 & 6.79 ± 0.48 & 31.71 ± 8.74 & 31.74 ± 8.74 \\
50 & HD 110879 & B2V+B3V & 3.31 & -0.178 &  & -2.097 & 0.034 & -1.7 & 3.417 ± 0.076 & 3.82 ± 0.26 & 8.94 ± 2.42 & 9.25 ± 2.43 \\
52 & HD 188252 & B2III & 5.91 & -0.174 & 896.22 & -2.066 & 0.044 & -3.98 & 4.316 ± 0.075 & 10.84 ± 0.76 & 15.36 ± 4.23 & 15.8 ± 4.25 \\
53 & HD 214263 & B2V & 6.84 & -0.131 & 510.1 & -1.976 & 0.073 & -1.93 & 3.456 ± 0.074 & 4.41 ± 0.25 & 7.81 ± 2.03 & 7.97 ± 2.03 \\
54 & HD 36960 & B0.5V & 4.78 & -0.248 &  & -2.821 & 0.022 & -3.2 & 4.303 ± 0.061 & 5.64 ± 0.36 & 15.16 ± 4.15 & 15.19 ± 4.15 \\
55 & HD 36285 & B2III & 6.33 & -0.194 & 353.96 & -2.157 & 0.024 & -1.49 & 3.353 ± 0.063 & 3.38 ± 0.18 & 7.64 ± 1.98 & 7.64 ± 1.98 \\
56 & HD 56139 & B2.5Ve & 4.01 & -0.15 & 204.85 & -1.879 & 0.054 & -3.4 & 4.006 ± 0.08 & 8.9 ± 0.62 & 12.17 ± 3.32 & 12.68 ± 3.34 \\
57 & HD 214993 & B2III & 5.25 & -0.137 & 386.44 & -2.412 & 0.101 & -3 & 4.061 ± 0.074 & 6 ± 0.45 & 6.11 ± 1.77 & 6.23 ± 1.77 \\
58 & HD 106490 & B2IV & 2.79 & -0.193 & 139.51 & -2.274 & 0.036 & -3.06 & 4.028 ± 0.104 & 6.62 ± 0.76 & 12.66 ± 4.26 & 13.4 ± 4.32 \\
59 & HD 184171 & B3IV & 4.74 & -0.15 & 226.52 & -1.443 & 0.026 & -2.21 & 3.357 ± 0.076 & 6.01 ± 0.41 & 5.16 ± 1.39 & 5.19 ± 1.39 \\
62 & HD 160578 & B1.5III & 2.39 & -0.171 &  & -2.224 & 0.054 & -3.63 & 4.239 ± 0.066 & 8.74 ± 0.53 & 17.37 ± 4.65 & 17.9 ± 4.66 \\
65 & HD 3360 & B2IV & 3.69 & -0.196 & 108.82 & -2.033 & 0.021 & -2.26 & 3.612 ± 0.074 & 5.01 ± 0.34 & 5.95 ± 1.61 & 5.96 ± 1.61 \\
66 & HD 16582 & B2IV & 4.08 & -0.212 &  & -2.094 & 0.014 & -2.42 & 3.701 ± 0.076 & 5.27 ± 0.39 & 6.61 ± 1.88 & 6.61 ± 1.88 \\
67 & HD 108249 & B1V & 1.58 & -0.17 &  & -2.57 & 0.075 & -2.86 & 4.068 ± 0.07 & 5.36 ± 0.37 & 10.78 ± 2.94 & 12.44 ± 3 \\
68 & HD 143275 & B0.3IV & 2.29 & -0.117 & 224 & -2.906 & 0.154 & -4.09 & 4.696 ± 0.132 & 8.31 ± 1.27 & 42.05 ± 17.2 & 43.21 ± 17.35 \\
69 & HD 214680 & O9V & 4.89 & -0.207 & 552 & -3.126 & 0.093 & -3.7 & 4.625 ± 0.073 & 6.12 ± 0.48 & 27.62 ± 7.91 & 27.69 ± 7.91 \\
70 & HD 93030 & B0Vp & 2.74 & -0.22 & 130.94 & -2.961 & 0.06 & -3.04 & 4.297 ± 0.1 & 4.93 ± 0.55 & 14.56 ± 4.82 & 14.82 ± 4.84 \\
71 & HD 37042 & B0.7V & 6.38 & -0.09 & 500 & -2.857 & 0.173 & -2.68 & 4.111 ± 0.071 & 4.43 ± 0.36 & 14.49 ± 2.9 & 14.51 ± 2.9 \\
72 & HD 37481 & B1.5IV & 5.96 & -0.216 & 364.78 & -2.324 & 0.018 & -1.91 & 3.588 ± 0.058 & 3.84 ± 0.2 & 8.18 ± 2.12 & 8.27 ± 2.13 \\
73 & HD 108248 & B0.5IV & 1.28 & -0.18 &  & -2.802 & 0.082 & -3.18 & 4.29 ± 0.068 & 5.65 ± 0.39 & 14.45 ± 4.01 & 14.67 ± 4.02 \\
74 & HD 34078 & O9.5V & 5.99 & 0.199 & 418 & -3.082 & 0.494 & -3.65 & 4.588 ± 0.056 & 6.05 ± 0.33 & 16.22 ± 4.35 & 16.24 ± 4.35 \\
75 & HD 36512 & O9.7V & 4.62 & -0.261 & 386 & -3.116 & 0.04 & -3.55 & 4.563 ± 0.069 & 5.75 ± 0.43 & 24.85 ± 7.02 & 24.87 ± 7.02 \\
77 & HD 24760 & B1.5III & 2.9 & -0.199 & 82.23 & -2.736 & 0.056 & -3.73 & 4.484 ± 0.068 & 7.54 ± 0.52 & 38.25 ± 10.38 & 38.89 ± 10.4 \\
78 & HD 74575 & B1.5III & 3.68 & -0.18 & 243.37 & -2.258 & 0.05 & -3.41 & 4.162 ± 0.06 & 7.69 ± 0.52 & 8.69 ± 1.58 & 8.69 ± 1.58 \\
80 & HD 50707 & B1IV & 4.82 & -0.212 &  & -2.542 & 0.037 & -3.16 & 4.175 ± 0.065 & 6.07 ± 0.39 & 5.52 ± 1.52 & 5.58 ± 1.53 \\
81 & HD 52089 & B1.5II & 1.5 & -0.211 &  & -2.249 & 0.023 & -4.04 & 4.412 ± 0.057 & 10.17 ± 0.55 & 8.07 ± 3.08 & 8.11 ± 3.08 \\
83 & HD 30836 & B2III & 3.68 & -0.157 & 248.08 & -2.098 & 0.064 & -3.59 & 4.169 ± 0.089 & 8.84 ± 0.82 & 6.6 ± 2.01 & 6.72 ± 2.02 \\
84 & HD 36591 & B1IV & 5.34 & -0.188 & 425.35 & -2.664 & 0.062 & -3.01 & 4.164 ± 0.088 & 5.55 ± 0.53 & 15.43 ± 4.74 & 15.43 ± 4.74 \\
85 & HD 205021 & B0.5IIIs & 3.23 & -0.201 &  & -2.658 & 0.051 & -3.54 & 4.377 ± 0.078 & 7.1 ± 0.58 & 21.33 ± 6.18 & 21.37 ± 6.18 \\
86 & HD 46328 & B0.7IV & 4.34 & -0.245 & 200.65 & -2.679 & 0.018 & -4.04 & 4.582 ± 0.071 & 8.67 ± 0.66 & 16.44 ± 6.55 & 16.44 ± 6.55 \\
89 & HD 35468 & B2V & 1.64 & -0.224 & 121 & -2.16 & 0.012 & -2.84 & 3.897 ± 0.063 & 6.15 ± 0.39 & 4.91 ± 2.55 & 4.99 ± 2.55 \\
90 & HD 51309 & B3Ib & 4.36 & -0.063 & 950 & -1.6 & 0.122 & -6.18 & 5.008 ± 0.198 & 35.71 ± 8.48 & 29.35 ± 20.11 & 29.54 ± 20.15 \\ \hline
\end{tabular}}
\end{table*}

==> old_tab_obs.tex <==
\begin{table*}[]
\caption{\textcolor{brown}{I will show this table in the "landscape" configuration, or I will split the table into two upon submission. For now, let's stick to this for our own sake.}List of our sample of stars. Mass, age, $\vini$, $\pev$, $\ptl$, $\ptg$, and $\pmax$ are the results from our Bayesian analysis (see text). The values of $\pev$, $\ptl$, $\ptg$, and $\pmax$ smaller than 0.05, 0.1, 0,1, and 0.6 are marked in red, respectively. \textcolor{brown}{Longitudinal magnetic field strengths are presented if the field is detected based on spectropolarimetric data. The underlined values in red highlight confirmed field detection in which all the corresponding references report field detection, while the plane values in red highlight uncertain field detection in which not all the corresponding references report field detection. When multiple values exist, we show the value with the highest significance.} If a star has spectropolarimetric data from \citet{Wade2016}, but it is insufficient to evaluate the star's magnetic properties, the field strength is not determined. Also shown is the information of known binaries. Most of the orbital periods ($P_\mathrm{orb}$) and eccentricities ($e$) for SB1/SB2 systems are obtained via SB9: The ninth catalog of spectroscopic binary orbits \citep{Pourbaix2004}. The maximum of the stellar radius over the Roche lobe radius $(R/R_\mathrm{RL})_\mathrm{max}$ is also shown (see text). Stars in NGC\,3293 are marked in bold. The luminosities of the stars that do not belong to NGC\,3293 are newly derived in this paper (see Table~\ref{tab_field}) \textcolor{red}{Ask Danny for details}}
\label{tab_obs}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccccccccccccccccccccc}
\hline \hline
No. & Star & $\logB$ & $\logC$ & $\logN$ & $\logO$ & \begin{tabular}[c]{@{}c@{}}$\Teff$\\ {[}K{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\logg$\\ {[}cm/s$^2${]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\logL$\\ {[}$\Lsun${}{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\vsini$\\ {[}km/s{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\veq$\\ {[}km/s{]}\end{tabular} & Ref. & \begin{tabular}[c]{@{}c@{}}Mass\\ {[}$\Msun${}{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Age\\ {[}Myr{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}$\vini$\\ {[}km/s{]}\end{tabular} & $\pev$ & $\ptl$ & $\ptg$ & $\pmax$ & \begin{tabular}[c]{@{}c@{}}$\langle B_\mathrm{l} \rangle$\\ {[}G{]}\end{tabular} & Ref. & Binary & \begin{tabular}[c]{@{}c@{}}$P_\mathrm{orb}$\\ {[}d{]}\end{tabular} & $e$ & Ref. & $(R/R_\mathrm{RL})_\mathrm{max}$ \\ \hline
1 & 44743 & 2.76 ± 0.20 & 8.16 ± 0.11 & 7.59 ± 0.14 & 8.62 ± 0.18 & 24.0 ± 1.0 & 3.50 ± 0.15 & 4.42 ± 0.06 & 23 & 1,2,3 & 12.1$^{+2.5}_{-2.5}$ & 13.5$^{+4.5}_{-3.2}$ & 45$^{+25}_{-25}$ & 0.54 / 0.80 / 0.60 / 0.99 & \$\prescript{\mathrm{m}}{(18,19,20,21,22)}{}\$-26 ± 3 \\
2 & 37023 & 2.74 ± 0.40 &  &  &  & 32.6 & 4.7 & 4.47 ± 0.07 & 57 & 1 & 16.0$^{+1.8}_{-1.8}}$ & 0.1$^{+0.3}_{-0.1}$ & 65$^{+25}_{-15}$ & \textcolor{red}{0.00} / 0.57 / \textcolor{red}{0.00} / 0.98 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(29)}{}\$SB2 / 20 / 0.68 / 0.6 \\
3 & 34816 & 2.71 ± 0.23 & 8.38 ± 0.05 & 7.81 ± 0.15 & 8.71 ± 0.09 & 30.4 & 4.3 & 4.35 ± 0.07 & 37 & 1,4,5 & 14.3$^{+2.2}_{-2.2}}$ & 0.2$^{+2.4}_{-0.2}$ & 45$^{+25}_{-15}$ & 0.20 / 0.81 / 0.29 / 0.83 &  \\
4 & 142669 & 2.71 ± 0.34 &  &  &  & 20.9 & 4.12 & 3.52 ± 0.06 & 103 & 5 & 7.3$^{+0.5}_{-1.2}}$ & 14.6$^{+9.3}_{-11.9}$ & 115$^{+25}_{-25}$ & 0.54 / 0.88 / 0.77 / 0.87 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(30)}{}\$SB1 / 4.0 / 0.27 / 0.6 \\
5 & 63578 & 2.69 ± 0.23 &  &  &  & 24.5 & 4.33 & 4.21 ± 0.08 & 84 & 5 & 9.0$^{+1.2}_{-0.7}}$ & 0.5$^{+4.8}_{-0.5}$ & 95$^{+25}_{-25}$ & \textcolor{red}{0.00} / 0.76 / 0.27 / 0.83 &  \\
6 & 112092 & 2.69 ± 0.40 &  &  &  & 20.5 & 4.3 & 3.32 ± 0.07 & 42 & 1 & 6.5$^{+0.9}_{-0.5}}$ & 1.2$^{+13.2}_{-1.2}$ & 55$^{+25}_{-25}$ & 0.31 / 0.81 / 0.41 / 0.87 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \\
7 & 212978 & 2.68 ± 0.30 &  &  &  & 19.9 & 3.91 & 3.69 ± 0.08 & 119 & 5 & 7.1$^{+1.0}_{-1.0}}$ & 26.8$^{+7.9}_{-7.9}$ & 135$^{+85}_{-25}$ & 0.43 / 0.76 / 0.63 / 0.78 &  \\
8 & 36351 & 2.64 ± 0.50 & 8.28 ± 0.04 & 7.68 ± 0.03 & 8.52 ± 0.06 & 22 & 4.16 & 3.66 ± 0.07 & 42 & 1,6 & 7.6$^{+0.7}_{-0.7}}$ & 11.5$^{+9.4}_{-11.5}$ & 55$^{+25}_{-25}$ & 0.32 / 0.86 / 0.82 / 0.80 &  \\
9 & 160762 & 2.63 ± 0.30 & 8.40 ± 0.07 & 7.89 ± 0.12 & 8.80 ± 0.09 & 17.5 & 3.8 & 3.40 ± 0.07 & 7.6 & 1,4,5 & 6.1$^{+0.5}_{-0.8}}$ & 46.4$^{+12.0}_{-12.0}$ & 15$^{+25}_{-15}$ & 0.77 / 0.76 / 0.62 / 0.68 & \$\prescript{\mathrm{m}}{(24)}{}\$Non-det. \$\prescript{\mathrm{b}}{(32)}{}\$SB1 / 114 / 0.43 / 0.1 \\
\textbf{10} & \textbf{3293-015} & \textbf{2.61 ± 0.21} &  & \textbf{7.98 ± 0.20} &  & \textbf{26.0 ± 1.5} & \textbf{3.80 ± 0.15} & \textbf{4.25 ± 0.07} & \textbf{294} & \textbf{7} & \textbf{13.4$^{+0.7}_{-0.7}$} & \textbf{2.7$^{+3.8}_{-2.7}$} & \textbf{305$^{+45}_{-45}$} & \textbf{0.57 / 0.79 / 0.54 / 0.75} &  \\
11 & 35039 & 2.60 ± 0.30 & 8.34 ± 0.10 & 7.77 ± 0.09 & 8.79 ± 0.07 & 19.6 ± 0.2 & 3.56 ± 0.07 & 3.90 ± 0.06 & 12 & 1,8 & 8.9$^{+0.8}_{-0.6}}$ & 25.9$^{+3.0}_{-2.2}$ & 25$^{+25}_{-25}$ & 0.55 / 0.90 / 0.86 / 0.88 &  \\
12 & 35299 & 2.59 ± 0.17 & 8.35 ± 0.09 & 7.82 ± 0.08 & 8.84 ± 0.09 & 23.5 & 4.2 & 3.70 ± 0.06 & 8.4 & 1,4,5 & 8.8$^{+0.7}_{-1.2}}$ & 7.0$^{+4.5}_{-7.0}$ & 15$^{+25}_{-15}$ & 0.58 / 0.87 / 0.70 / \textcolor{red}{0.42} &  \\
13 & BD+56 576 & 2.59 ± 0.14 & 7.84 ± 0.18 & 7.62 ± 0.22 & 8.34 ± 0.14 & 22.5 & 3.55 & 4.39 ± 0.07 & 27 & 5,6 & 11.2$^{+2.5}_{-2.5}}$ & 17.3$^{+4.6}_{-4.6}$ & 45$^{+35}_{-25}$ & 0.66 / 0.85 / 0.66 / 0.89 &  \\
\textbf{14} & \textbf{3293-023} & \textbf{2.59 ± 0.26} & \textbf{7.72 ± 0.25} & \textbf{7.65 ± 0.23} & \textbf{8.69 ± 0.36} & \textbf{22.7 ± 1.0} & \textbf{3.90 ± 0.10} & \textbf{3.75 ± 0.06} & \textbf{169} & \textbf{7,9} & \textbf{9.0$^{+0.4}_{-0.4}$} & \textbf{16.2$^{+6.0}_{-6.0}$} & \textbf{205$^{+25}_{-35}$} & \textbf{0.35 / 0.87 / 0.64 / 0.92} &  \\
15 & 121790 & 2.58 ± 0.32 &  &  &  & 21.4 & 4.15 & 3.45 ± 0.06 & 119 & 5 & 7.4$^{+1.3}_{-0.5}}$ & 10.1$^{+10.1}_{-10.1}$ & 135$^{+95}_{-25}$ & 0.85 / 0.85 / 0.83 / 1.02 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \\
16 & 36430 & 2.53 ± 0.50 & 8.38 ± 0.03 & 7.67 ± 0.09 & 8.57 ± 0.04 & 19.6 & 4.36 & 3.39 ± 0.07 & 26 & 1,6 & 6.1$^{+0.5}_{-0.5}}$ & 1.3$^{+11.4}_{-1.3}$ & 35$^{+25}_{-25}$ & \textcolor{red}{0.02} / 0.85 / 0.24 / 0.65 &  \\
17 & 64722 & 2.52 ± 0.32 &  &  &  & 24.8 & 4.05 & 3.95 ± 0.06 & 124 & 5 & 10.2$^{+1.4}_{-1.4}}$ & 9.7$^{+4.6}_{-5.6}$ & 185$^{+45}_{-65}$ & 0.85 / 0.90 / 0.72 / 0.86 &  \\
18 & 36959 & 2.51 ± 0.20 & 8.37 ± 0.11 & 7.85 ± 0.09 & 8.70 ± 0.06 & 26.1 ± 0.2 & 4.25 ± 0.07 & 3.80 ± 0.05 & 12 & 1,8 & 10.7$^{+0.5}_{-0.8}}$ & 1.5$^{+3.7}_{-1.5}$ & 25$^{+25}_{-25}$ & 0.48 / 0.49 / 0.60 / \textcolor{red}{0.46} & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \\
19 & 37744 & 2.51 ± 0.60 & 8.32 ± 0.07 & 7.81 ± 0.10 & 8.70 ± 0.07 & 24.0 ± 0.4 & 4.10 ± 0.10 & 3.61 ± 0.05 & 33 & 1,8 & 9.4$^{+0.4}_{-0.4}}$ & 9.4$^{+5.9}_{-4.5}$ & 45$^{+35}_{-25}$ & 0.13 / 0.59 / 0.86 / 0.83 &  \\
\textbf{20} & \textbf{3293-038} & \textbf{2.50 ± 0.22} & \textbf{8.16 ± 0.26} & \textbf{7.34 ± 0.29} & \textbf{8.61 ± 0.41} & \textbf{20.2 ± 1.0} & \textbf{3.95 ± 0.15} & \textbf{3.29 ± 0.07} & \textbf{229} & \textbf{7} & \textbf{6.9$^{+0.5}_{-0.5}$} & \textbf{10.2$^{+13.1}_{-10.2}$} & \textbf{255$^{+55}_{-35}$} & \textbf{0.23 / 0.82 / 0.58 / 0.83} &  \\
21 & 37017 & 2.50 ± 0.38 &  &  &  & 19 & 4.2 & 3.17 ± 0.08 & 140 & 5 & 5.7$^{+0.5}_{-0.5}}$ & 14.1$^{+14.1}_{-14.1}$ & 185$^{+45}_{-35}$ & 0.60 / 0.85 / 0.73 / 0.91 & \$\prescript{\mathrm{m}}{(22)}{}\$-1800 ± 300 \$\prescript{\mathrm{b}}{(34)}{}\$SB1 / 19 / 0.31 / 0.2 \\
22 & 122980 & 2.50 ± 0.30 & 8.32 ± 0.09 & 7.76 ± 0.08 & 8.72 ± 0.06 & 20.8 ± 0.3 & 4.22 ± 0.05 & 3.37 ± 0.04 & 18 & 1,4 & 7.0$^{+0.4}_{-0.6}}$ & 10.1$^{+5.9}_{-6.9}$ & 25$^{+25}_{-25}$ & 0.34 / 0.95 / 0.85 / \textcolor{red}{0.39} & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \\
23 & 37209 & 2.48 ± 0.60 & 8.19 ± 0.04 & 7.56 ± 0.05 & 8.51 ± 0.08 & 24.1 & 4.13 & 3.78 ± 0.06 & 50 & 1,6 & 8.8$^{+1.7}_{-0.7}}$ & 9.6$^{+5.8}_{-7.1}$ & 65$^{+25}_{-25}$ & 0.87 / 0.88 / 0.83 / 0.73 &  \\
24 & 111123 & 2.48 ± 0.20 & 8.04 ± 0.10 & 7.61 ± 0.17 & 8.59 ± 0.16 & 27.5 ± 1.0 & 3.65 ± 0.20 & 4.36 ± 0.09 & 48 & 1,10,11 & 13.6$^{+3.3}_{-2.4}}$ & 9.4$^{+2.3}_{-1.6}$ & 35$^{+15}_{-25}$ & 0.20 / 0.78 / 0.50 / \textcolor{red}{0.02} & \$\prescript{\mathrm{m}}{(20,21)}{}\$Non-det. \$\prescript{\mathrm{b}}{(35)}{}\$SB1 / 1828 / 0.38 / 0.0 \\
25 & 36629 & 2.47 ± 0.30 & 8.32 ± 0.03 & 7.61 ± 0.03 & 8.32 ± 0.06 & 22.3 & 4.35 & 3.27 ± 0.07 & 4.1 & 1,6 & 7.6$^{+0.7}_{-0.7}}$ & 0.8$^{+7.3}_{-0.8}$ & 15$^{+15}_{-15}$ & 0.10 / 0.19 / 0.24 / \textcolor{red}{0.45} & \$\prescript{\mathrm{m}}{(21)}{}\$Non-det. \\
26 & 37020 & 2.47 ± 0.40 & 8.40 ± 0.07 & 7.85 ± 0.09 & 8.70 ± 0.10 & 30.7 ± 0.3 & 4.30 ± 0.08 & 4.29 ± 0.08 & 45 & 1,8 & 14.7$^{+0.9}_{-0.9}}$ & 0.1$^{+1.5}_{-0.1}$ & 55$^{+25}_{-25}$ & 0.28 / 0.58 / 0.29 / 0.65 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(36)}{}\$SB1 / 65 / 0.63 / 0.2 \\
\textbf{27} & \textbf{3293-012} & \textbf{2.46 ± 0.26} & \textbf{7.86 ± 0.17} & \textbf{7.47 ± 0.13} & \textbf{8.83 ± 0.25} & \textbf{24.5 ± 1.0} & \textbf{3.70 ± 0.10} & \textbf{4.35 ± 0.06} & \textbf{102} & \textbf{7,9} & \textbf{12.1$^{+1.3}_{-0.6}$} & \textbf{13.4$^{+2.2}_{-2.2}$} & \textbf{125$^{+25}_{-25}$} & \textbf{0.79 / 0.80 / 0.69 / 0.78} &  \\
28 & 37356 & 2.46 ± 0.40 & 8.41 ± 0.03 & 7.70 ± 0.04 & 8.44 ± 0.05 & 22.4 & 4.13 & 3.93 ± 0.08 & 23 & 1,6 & 7.6$^{+1.7}_{-0.7}}$ & 10.6$^{+10.6}_{-6.8}$ & 35$^{+25}_{-25}$ & 0.06 / 0.76 / 0.80 / \textcolor{red}{0.51} &  \\
29 & 41753 & 2.46 ± 0.50 & 8.53 ± 0.15 & 8.10 ± 0.14 & 8.57 ± 0.05 & 17.1 & 3.94 & 3.31 ± 0.08 & 49 & 1,6 & 5.1$^{+0.4}_{-0.1}}$ & 46.4$^{+15.5}_{-12.0}$ & 65$^{+25}_{-25}$ & 0.37 / 0.75 / 0.71 / 0.78 &  \\
30 & 109668 & 2.46 ± 0.33 &  &  &  & 21.4 & 4.06 & 3.85 ± 0.11 & 118 & 5 & 7.6$^{+1.0}_{-1.0}}$ & 16.9$^{+7.9}_{-10.2}$ & 185$^{+55}_{-75}$ & 0.13 / 0.71 / 0.70 / 0.84 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(31)}{}\$SB2 / --- / --- / --- \\
31 & 29248 & 2.45 ± 0.40 & 8.29 ± 0.13 & 7.93 ± 0.09 & 8.78 ± 0.09 & 22.0 ± 0.3 & 3.85 ± 0.05 & 3.86 ± 0.06 & 26 & 1,4,12 & 8.9$^{+0.5}_{-0.4}}$ & 20.9$^{+1.0}_{-1.5}$ & 25$^{+15}_{-15}$ & 0.75 / 0.86 / 0.84 / \textcolor{red}{0.18} & \$\prescript{\mathrm{m}}{(18,20,21,25)}{}\$Non-det. \\
32 & 38622 & 2.45 ± 0.37 &  &  &  & 17.5 & 3.59 & 3.39 ± 0.08 & 48 & 5 & 7.4$^{+0.7}_{-1.5}}$ & 39.5$^{+15.5}_{-8.6}$ & 75$^{+25}_{-25}$ & 0.20 / 0.75 / 0.62 / 0.94 &  \\
33 & 120324 & 2.44 ± 0.31 &  &  &  & 22.5 & 3.75 & 3.74 ± 0.09 & 159 & 5 & 9.8$^{+1.1}_{-1.8}}$ & 18.0$^{+6.0}_{-4.3}$ & 205$^{+35}_{-35}$ & 0.09 / 0.83 / 0.64 / 0.86 & \$\prescript{\mathrm{m}}{(21,26)}{}\$Non-det. \\
34 & 202347 & 2.44 ± 0.32 &  &  &  & 23.3 & 4.13 & 3.74 ± 0.07 & 118 & 5 & 8.8$^{+1.2}_{-0.7}}$ & 9.9$^{+5.3}_{-8.3}$ & 185$^{+55}_{-75}$ & 0.70 / 0.90 / 0.82 / 0.92 &  \\
35 & 64740 & 2.43 ± 0.30 &  &  &  & 22.8 & 4.1 & 3.74 ± 0.06 & 131 & 5 & 8.6$^{+0.7}_{-1.2}}$ & 12.1$^{+5.7}_{-8.9}$ & 185$^{+45}_{-45}$ & 0.59 / 0.88 / 0.76 / 0.86 & \$\prescript{\mathrm{m}}{(22)}{}\$-820 ± 90 \\
36 & 68243 & 2.43 ± 0.19 &  &  &  & 24.3 & 3.92 & 4.43 ± 0.07 & 93 & 5 & 9.9$^{+1.7}_{-1.7}}$ & 13.4$^{+4.1}_{-2.9}$ & 115$^{+25}_{-25}$ & \textcolor{red}{0.03} / 0.78 / 0.66 / 0.86 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(38)}{}\$SB1 / 1.5 / 0.06 / 1.7 \\
37 & 45546 & 2.42 ± 0.29 &  &  &  & 19.4 & 3.76 & 3.44 ± 0.09 & 60 & 5 & 7.0$^{+1.1}_{-0.7}}$ & 30.2$^{+11.1}_{-7.9}$ & 85$^{+25}_{-25}$ & 0.20 / 0.78 / 0.62 / 0.95 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \\
38 & 24131 & 2.38 ± 0.22 &  &  &  & 26.4 & 4.36 & 4.02 ± 0.06 & 75 & 5 & 10.8$^{+1.4}_{-1.9}}$ & 0.4$^{+2.7}_{-0.4}$ & 85$^{+25}_{-25}$ & 0.06 / 0.88 / 0.17 / \textcolor{red}{0.41} &  \\
\textbf{39} & \textbf{3293-030} & \textbf{2.36 ± 0.21} & \textbf{7.86 ± 0.27} & \textbf{7.67 ± 0.27} & \textbf{8.65 ± 0.37} & \textbf{19.8 ± 1.0} & \textbf{3.80 ± 0.15} & \textbf{3.41 ± 0.08} & \textbf{215} & \textbf{7} & \textbf{7.1$^{+0.4}_{-0.4}$} & \textbf{23.6$^{+11.0}_{-11.0}$} & \textbf{245$^{+45}_{-45}$} & \textbf{0.24 / 0.85 / 0.53 / 0.90} &  \\
40 & 886 & 2.35 ± 0.19 & 8.37 ± 0.08 & 7.76 ± 0.07 & 8.73 ± 0.11 & 22 & 3.95 & 3.99 ± 0.08 & 10 & 1,4,5 & 8.2$^{+1.2}_{-0.7}}$ & 19.8$^{+5.2}_{-5.2}$ & 25$^{+25}_{-25}$ & 0.18 / 0.76 / 0.65 / \textcolor{red}{0.23} & \$\prescript{\mathrm{m}}{(18,24,27)}{}\$46 ± 11 \$\prescript{\mathrm{b}}{(25)}{}\$SB1 / 6.8 / --- / \textgreater{} 0.5 \\
41 & 143018 & 2.34 ± 0.35 &  &  &  & 27.5 & 4.2 & 3.94 ± 0.09 & 107 & 5 & 11.7$^{+1.4}_{-1.4}}$ & 2.9$^{+4.2}_{-2.9}$ & 115$^{+35}_{-15}$ & 0.43 / 0.41 / 0.67 / 0.69 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(39)}{}\$SB2,EB / 1.6 / 0.0 / 0.7 \\
42 & 216916 & 2.32 ± 0.16 & 8.32 ± 0.07 & 7.78 ± 0.10 & 8.78 ± 0.08 & 23 & 3.95 & 3.97 ± 0.07 & 15 & 1,4,5 & 9.2$^{+1.4}_{-1.4}}$ & 16.9$^{+4.0}_{-4.0}$ & 25$^{+25}_{-25}$ & 0.51 / 0.78 / 0.65 / \textcolor{red}{0.25} & \$\prescript{\mathrm{m}}{(18)}{}\$Non-det. \$\prescript{\mathrm{b}}{(40)}{}\$EB / 12 / 0.05 / 0.3 \\
43 & 121743 & 2.30 ± 0.29 &  &  &  & 21.6 & 4.08 & 3.53 ± 0.06 & 68 & 5 & 7.6$^{+1.0}_{-1.0}}$ & 16.9$^{+7.9}_{-7.9}$ & 85$^{+25}_{-25}$ & 0.78 / 0.90 / 0.72 / 0.63 & \$\prescript{\mathrm{m}}{(22)}{}\$330 ± 90 \\
44 & 35337 & 2.27 ± 0.17 & 8.31 ± 0.09 & 7.64 ± 0.10 & 8.55 ± 0.17 & 23.6 & 4.2 & 3.90 ± 0.06 & 15 & 1,5,6 & 8.9$^{+0.7}_{-1.7}}$ & 6.9$^{+5.7}_{-6.9}$ & 25$^{+25}_{-25}$ & 0.12 / 0.83 / 0.70 / \textcolor{red}{0.14} &  \\
\textbf{45} & \textbf{3293-024} & \textbf{2.24 ± 0.25} & \textbf{7.75 ± 0.23} & \textbf{7.6 ± 0.25} & \textbf{8.78 ± 0.35} & \textbf{22.2 ± 1.0} & \textbf{3.85 ± 0.10} & \textbf{3.75 ± 0.06} & \textbf{151} & \textbf{7,9} & \textbf{8.9$^{+0.4}_{-0.4}$} & \textbf{19.3$^{+6.4}_{-4.6}$} & \textbf{195$^{+35}_{-35}$} & \textbf{0.34 / 0.82 / 0.64 / 0.86} &  \\
\textbf{46} & \textbf{3293-019} & \textbf{2.23 ± 0.30} & \textbf{8.26 ± 0.29} & \textbf{7.57 ± 0.25} & \textbf{8.58 ± 0.24} & \textbf{25.0 ± 1.0} & \textbf{3.85 ± 0.10} & \textbf{4.13 ± 0.06} & \textbf{129} & \textbf{7,9} & \textbf{11.4$^{+0.5}_{-0.9}$} & \textbf{13.3$^{+2.5}_{-3.4}$} & \textbf{185$^{+35}_{-45}$} & \textbf{0.63 / 0.81 / 0.68 / 0.80} &  \\
\textbf{47} & \textbf{3293-028} & \textbf{2.22 ± 0.22} & \textbf{7.69 ± 0.33} & \textbf{7.56 ± 0.30} & \textbf{8.69 ± 0.43} & \textbf{21.2 ± 1.0} & \textbf{3.90 ± 0.15} & \textbf{3.65 ± 0.07} & \textbf{222} & \textbf{7} & \textbf{8.3$^{+0.4}_{-0.4}$} & \textbf{17.0$^{+8.0}_{-8.0}$} & \textbf{255$^{+45}_{-35}$} & \textbf{0.64 / 0.80 / 0.57 / 0.68} &  \\
48 & 180163 & 2.21 ± 0.60 &  &  &  & 16.5 & 3.27 & 3.82 ± 0.08 & 37 & 1 & 6.7$^{+1.8}_{-1.1}}$ & 36.9$^{+17.8}_{-8.1}$ & 65$^{+25}_{-25}$ & 0.09 / 0.28 / 0.11 / \textcolor{red}{0.48} &  \\
49 & 22951 & 2.19 ± 0.17 & 8.11 ± 0.21 & 7.69 ± 0.32 & 8.42 ± 0.17 & 28 & 4.26 & 4.40 ± 0.07 & 30 & 1,5,6 & 12.2$^{+1.4}_{-1.4}}$ & 1.5$^{+4.5}_{-1.5}$ & 45$^{+25}_{-25}$ & \textcolor{red}{0.02} / 0.80 / 0.46 / \textcolor{red}{0.34} &  \\
50 & 110879 & 2.17 ± 0.38 &  &  &  & 21.2 & 4.21 & 3.42 ± 0.08 & 125 & 5 & 7.3$^{+0.5}_{-0.9}}$ & 9.2$^{+9.2}_{-9.2}$ & 185$^{+65}_{-65}$ & 0.66 / 0.84 / 0.69 / 0.78 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(31)}{}\$SB2 / --- / --- / --- \\
\textbf{51} & \textbf{3293-031} & \textbf{2.16 ± 0.22} & \textbf{7.66 ± 0.33} & \textbf{7.57 ± 0.37} &  & \textbf{21.0 ± 1.0} & \textbf{4.00 ± 0.15} & \textbf{3.51 ± 0.07} & \textbf{265} & \textbf{7} & \textbf{7.7$^{+0.4}_{-0.4}$} & \textbf{14.8$^{+8.0}_{-8.0}$} & \textbf{305$^{+35}_{-45}$} & \textbf{0.67 / 0.91 / 0.63 / 0.81} &  \\
52 & 188252 & 2.10 ± 0.25 &  &  &  & 21.1 & 3.54 & 4.32 ± 0.08 & 88 & 5 & 10.0$^{+2.3}_{-2.3}}$ & 20.8$^{+6.1}_{-6.1}$ & 185$^{+45}_{-75}$ & 0.39 / 0.74 / 0.66 / 0.91 &  \\
53 & 214263 & 2.06 ± 0.36 &  &  &  & 20.2 & 4.03 & 3.46 ± 0.07 & 84 & 5 & 6.9$^{+0.9}_{-0.9}}$ & 23.5$^{+7.8}_{-11.0}$ & 95$^{+35}_{-25}$ & 0.81 / 0.85 / 0.66 / 0.73 &  \\
54 & 36960 & 2.02 ± 0.25 & 8.35 ± 0.09 & 7.72 ± 0.11 & 8.67 ± 0.08 & 29 & 4.1 & 4.30 ± 0.06 & 34 & 1,4,5 & 14.4$^{+1.4}_{-3.2}}$ & 5.4$^{+2.3}_{-2.8}$ & 45$^{+35}_{-15}$ & 0.91 / 0.91 / 0.83 / \textcolor{red}{0.34} & \$\prescript{\mathrm{m}}{(21)}{}\$Non-det. \\
55 & 36285 & 1.99 ± 0.19 & 8.32 ± 0.07 & 7.77 ± 0.09 & 8.80 ± 0.10 & 21.7 & 4.25 & 3.35 ± 0.06 & 12 & 1,5,8 & 7.3$^{+0.9}_{-0.9}}$ & 4.6$^{+10.1}_{-4.6}$ & 25$^{+25}_{-25}$ & 0.48 / 0.53 / 0.56 / \textcolor{red}{0.07} &  \\
56 & 56139 & 1.97 ± 0.37 &  &  &  & 19.5 & 3.61 & 4.01 ± 0.08 & 105 & 5 & 8.3$^{+1.5}_{-1.5}}$ & 27.0$^{+7.9}_{-7.9}$ & 185$^{+55}_{-25}$ & 0.46 / 0.72 / 0.65 / 0.89 & \$\prescript{\mathrm{m}}{(21)}{}\$Non-det. \\
57 & 214993 & 1.94 ± 0.19 & 8.22 ± 0.12 & 7.64 ± 0.18 & 8.42 ± 0.23 & 24.5 & 3.65 & 4.06 ± 0.07 & 62 & 1,2,5,13 & 11.9$^{+2.4}_{-2.4}}$ & 13.4$^{+4.1}_{-2.9}$ & 85$^{+25}_{-25}$ & 0.06 / 0.78 / 0.70 / \textcolor{red}{0.44} & \$\prescript{\mathrm{m}}{(18)}{}\$Non-det. \\
58 & 106490 & 1.89 ± 0.33 &  &  &  & 22.9 & 3.88 & 4.03 ± 0.10 & 147 & 5 & 9.6$^{+1.5}_{-1.5}}$ & 16.9$^{+4.0}_{-5.6}$ & 205$^{+45}_{-35}$ & 0.60 / 0.71 / 0.64 / 0.83 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \\
59 & 184171 & 1.84 ± 0.70 & 8.28 ± 0.13 & 7.86 ± 0.25 & 8.69 ± 0.05 & 16.3 & 3.58 & 3.36 ± 0.08 & 31 & 1,6 & 6.3$^{+0.5}_{-0.5}}$ & 53.3$^{+12.0}_{-15.5}$ & 55$^{+25}_{-25}$ & 0.48 / 0.74 / 0.59 / \textcolor{red}{0.48} &  \\
\textbf{60} & \textbf{3293-008} & \textbf{1.84 ± 0.26} & \textbf{7.83 ± 0.23} & \textbf{7.55 ± 0.15} & \textbf{8.77 ± 0.32} & \textbf{23.6 ± 1.0} & \textbf{3.40 ± 0.10} & \textbf{4.43 ± 0.06} & \textbf{138} & \textbf{7,9} & \textbf{12.6$^{+0.7}_{-0.7}$} & \textbf{14.0$^{+1.6}_{-1.6}$} & \textbf{205$^{+35}_{-25}$} & \textbf{0.23 / 0.83 / 0.70 / 0.83} &  \\
\textbf{61} & \textbf{3293-004} & \textbf{1.74 ± 0.25} & \textbf{8.17 ± 0.28} & \textbf{7.57 ± 0.09} & \textbf{8.75 ± 0.19} & \textbf{24.0 ± 1.0} & \textbf{3.04 ± 0.10} & \textbf{4.64 ± 0.06} & \textbf{100} & \textbf{7,9} & \textbf{14.4$^{+0.9}_{-0.7}$} & \textbf{12.3$^{+1.3}_{-0.9}$} & \textbf{195$^{+35}_{-25}$} & \textbf{\textcolor{red}{0.00} / 0.84 / 0.60 / 0.76} &  \\
62 & 160578 & 1.64 ± 0.39 &  &  &  & 22.5 & 3.78 & 4.24 ± 0.07 & 108 & 5 & 10.2$^{+1.0}_{-2.4}}$ & 17.3$^{+4.6}_{-4.6}$ & 205$^{+115}_{-45}$ & 0.20 / 0.82 / 0.64 / 0.90 & \$\prescript{\mathrm{m}}{(19,21)}{}\$Non-det. \\
\textbf{63} & \textbf{3293-010} & \textbf{1.53 ± 0.33} & \textbf{7.85 ± 0.21} & \textbf{7.59 ± 0.08} & \textbf{8.82 ± 0.23} & \textbf{23.6 ± 1.0} & \textbf{3.55 ± 0.10} & \textbf{4.31 ± 0.06} & \textbf{73} & \textbf{7,9} & \textbf{11.8$^{+0.7}_{-0.7}$} & \textbf{14.8$^{+2.4}_{-1.4}$} & \textbf{205$^{+45}_{-35}$} & \textbf{0.41 / 0.80 / 0.69 / 0.76} &  \\
\textbf{64} & \textbf{3293-005} & \textbf{1.50 ± 0.28} & \textbf{7.89 ± 0.24} & \textbf{7.59 ± 0.08} & \textbf{8.75 ± 0.30} & \textbf{22.6 ± 1.5} & \textbf{3.00 ± 0.10} & \textbf{4.60 ± 0.08} & \textbf{184} & \textbf{7} & \textbf{13.5$^{+1.2}_{-1.2}$} & \textbf{13.7$^{+1.8}_{-2.3}$} & \textbf{275$^{+45}_{-45}$} & \textbf{\textcolor{red}{0.01} / 0.70 / 0.72 / \textcolor{red}{0.05}} &  \\
65 & 3360 & 1.18 ± 0.17 & 8.31 ± 0.08 & 8.23 ± 0.07 & 8.80 ± 0.08 & 20.7 & 3.8 & 3.61 ± 0.07 & 21 & 1,4,5,14 & 9.9$^{+1.3}_{-1.3}}$ & 20.6$^{+6.0}_{-6.0}$ & 185$^{+45}_{-25}$ & 0.31 / 0.79 / 0.63 / \textcolor{red}{0.20} & \$\prescript{\mathrm{m}}{(14,22,24)}{}\$-20 ± 4 \\
66 & 16582 & 1.08 ± 0.15 & 8.21 ± 0.09 & 8.23 ± 0.08 & 8.79 ± 0.07 & 21.3 & 3.8 & 3.70 ± 0.08 & 14 & 1,4,5,15 & 11.2$^{+1.1}_{-1.1}}$ & 17.6$^{+3.6}_{-2.8}$ & 125$^{+25}_{-15}$ & 0.36 / 0.78 / 0.63 / \textcolor{red}{0.00} & \$\prescript{\mathrm{m}}{(18,20,21,24,26)}{}\$-75 ± 14 \\
67 & 108249 & 2.98 &  &  &  & 26 & 4 & 4.07 ± 0.07 & 244 & 5 & 12.5$^{+2.3}_{-1.6}}$ & 9.5$^{+2.7}_{-2.7}$ & 325$^{+115}_{-45}$ & 0.68 / 0.90 / 0.69 /  0.88 &  \\
68 & 143275 & 2.75 &  &  &  & 30.1 & 4.2 & 4.70 ± 0.13 & 163 & 5 & 14.2$^{+2.2}_{-1.4}}$ & 1.6$^{+2.9}_{-1.6}$ & 185$^{+45}_{-25}$ & \textcolor{red}{0.04} / 0.70 / 0.65 / 0.91 & \$\prescript{\mathrm{m}}{(18)}{}\$Non-det. \$\prescript{\mathrm{b}}{(41)}{}\$SB1 / 3864 / 0.94 / 0.1 \\
69 & 214680 & 2.70 &  &  &  & 33.6 & 4.29 & 4.63 ± 0.07 & 46 & 1 & 18.4$^{+2.2}_{-3.1}}$ & 0.1$^{+1.6}_{-0.1}$ & 55$^{+25}_{-15}$ & 0.23 / 0.78 / 0.29 /  0.84 & \$\prescript{\mathrm{m}}{(24)}{}\$204 ± 55 \\
70 & 93030 & 2.65 &  &  &  & 31 & 4.2 & 4.30 ± 0.10 & 101 & 5 & 14.8$^{+3.1}_{-1.3}}$ & 1.0$^{+3.0}_{-1.0}$ & 115$^{+25}_{-25}$ & 0.46 / 0.47 / 0.64 /  1.26 & \$\prescript{\mathrm{m}}{(21)}{}\$Non-det. \$\prescript{\mathrm{b}}{(42)}{}\$SB1 / 2.2 / --- / \textgreater{} 0.6 \\
71 & 37042 & 2.54 & 8.33 ± 0.11 & 8.04 ± 0.08 & 8.75 ± 0.08 & 29.3 ± 0.3 & 4.30 ± 0.05 & 4.11 ± 0.07 & 30 & 1,8 & 13.3$^{+0.6}_{-0.9}$ & 0.1$^{+1.1}_{-0.1}$ & 35$^{+35}_{-15}$ & 0.22 / 0.41 / 0.27 /  0.72 & \$\prescript{\mathrm{m}}{(24)}{}\$Non-det. \\
72 & 37481 & 2.47 & 8.39 & 7.55 ± 0.02 & 8.75 ± 0.08 & 23.3 & 4.17 & 3.59 ± 0.06 & 67 & 1,6 & 8.8$^{+0.7}_{-1.7}$ & 8.6$^{+7.3}_{-8.6}$ & 85$^{+25}_{-25}$ & 0.68 / 0.66 / 0.78 /  0.62 &  \\
73 & 108248 & 2.31 &  &  &  & 28.8 & 4.08 & 4.29 ± 0.07 & 85 & 5 & 15.2$^{+1.4}_{-3.3}$ & 6.1$^{+1.9}_{-1.9}$ & 295$^{+35}_{-35}$ & 0.86 / 0.91 / 0.79 /  0.78 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \\
74 & 34078 & 2.2 &  & 7.25 ± 0.09 & 8.34 ± 0.25 & 33 & 4.07 & 4.59 ± 0.06 & 24 & 1,5,16 & 18.9$^{+3.1}_{-2.2}$ & 4.3$^{+1.1}_{-1.4}$ & 35$^{+25}_{-25}$ & 0.50 / 0.83 / 0.82 / \textcolor{red}{0.36} & \$\prescript{\mathrm{m}}{(24,28)}{}\$Non-det. \\
75 & 36512 & 2.2 & 8.35 ± 0.14 & 7.79 ± 0.11 & 8.75 ± 0.09 & 33.4 & 4.3 & 4.56 ± 0.07 & 25 & 1,4,5 & 18.4$^{+1.3}_{-3.1}$ & 0.2$^{+1.7}_{-0.2}$ & 35$^{+25}_{-25}$ & 0.26 / 0.64 / 0.26 / \textcolor{red}{0.19} &  \\
\textbf{76} & \textbf{3293-016} & \textbf{ 2.0} &  & \textbf{7.66 ± 0.15} &  & \textbf{25.3 ± 1.0} & \textbf{3.80 ± 0.10} & \textbf{4.18 ± 0.06} & \textbf{54} & \textbf{7} & \textbf{12.1$^{+0.6}_{-1.0}$} & \textbf{11.8$^{+2.4}_{-3.3}$} & \textbf{385$^{+55}_{-75}$} & \textbf{0.45 / 0.82 / 0.68 / 0.95} &  \\
77 & 24760 & 2.04 &  &  &  & 27.8 & 4.25 & 4.48 ± 0.07 & 128 & 5 & 12.5$^{+1.4}_{-2.0}$ & 3.4$^{+3.4}_{-3.4}$ & 185$^{+65}_{-55}$ & \textcolor{red}{0.01} / 0.81 / 0.49 / 0.68 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(44)}{}\$SB1 / 14 / 0.46 / 0.5 \\
78 & 74575 & 1.84 & 8.37 ± 0.10 & 7.92 ± 0.10 & 8.79 ± 0.08 & 22.9 ± 0.3 & 3.60 ± 0.05 & 4.16 ± 0.06 & 11 & 1,4 & 12.1$^{+0.4}_{-1.2}$ & 15.5$^{+1.5}_{-1.1}$ & 215$^{+65}_{-45}$ & 0.13 / 0.85 / 0.85 / \textcolor{red}{ 0.37} & \$\prescript{\mathrm{m}}{(20,21,26)}{}\$-219 ± 60 \\
\textbf{79} & \textbf{3293-007} & \textbf{ 1.8} & \textbf{8.13 ± 0.22} & \textbf{7.66 ± 0.08} & \textbf{8.71 ± 0.17} & \textbf{23.2 ± 1.0} & \textbf{3.08 ± 0.10} & \textbf{4.69 ± 0.06} & \textbf{56} & \textbf{7,9} & \textbf{14.9$^{+1.0}_{-0.7}$} & \textbf{12.1$^{+1.0}_{-1.0}$} & \textbf{205$^{+55}_{-35}$} & \textbf{\textcolor{red}{0.05} / 0.88 / 0.65 / 0.75} &  \\
80 & 50707 & 1.64 & 8.18 ± 0.10 & 8.03 ± 0.15 & 8.64 ± 0.18 & 26 & 3.6 & 4.18 ± 0.07 & 44 & 1,5,11 & 14.8$^{+2.3}_{-2.3}$ & 10.5$^{+1.9}_{-2.7}$ & 335$^{+55}_{-45}$ & \textcolor{red}{0.02} / 0.83 / 0.67 / 1.03 & \$\prescript{\mathrm{m}}{(20,21,26)}{}\$149 ± 19 \\
81 & 52089 & 1.62 & 8.09 ± 0.12 & 7.93 ± 0.14 & 8.44 ± 0.18 & 23.0 ± 1.0 & 3.30 ± 0.15 & 4.41 ± 0.06 & 28 & 1,11 & 14.5$^{+4.4}_{-3.4}$ & 10.6$^{+5.0}_{-3.6}$ & 325$^{+65}_{-35}$ & 0.19 / 0.86 / 0.59 /  0.87 & \$\prescript{\mathrm{m}}{(20,21,22,26)}{}\$-156 ± 18 \\
\textbf{82} & \textbf{3293-006} & \textbf{ 1.6} & \textbf{7.81 ± 0.23} & \textbf{7.57 ± 0.16} & \textbf{8.84 ± 0.31} & \textbf{24.0 ± 1.5} & \textbf{3.15 ± 0.10} & \textbf{4.61 ± 0.07} & \textbf{211} & \textbf{7} & \textbf{14.2$^{+1.6}_{-1.2}$} & \textbf{11.8$^{+1.8}_{-1.8}$} & \textbf{415$^{+75}_{-45}$} & \textbf{\textcolor{red}{0.05} / 0.78 / 0.61 / \textcolor{red}{ 0.28}} &  \\
83 & 30836 & 1.50 & 8.19 ± 0.09 & 7.54 ± 0.15 & 8.40 ± 0.29 & 21.5 & 3.35 & 4.17 ± 0.09 & 51 & 1,5,11 & 12.2$^{+2.5}_{-2.5}$ & 16.0$^{+5.3}_{-5.3}$ & 205$^{+55}_{-35}$ & 0.12 / 0.79 / 0.66 /  0.68 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(45)}{}\$SB1 / 9.5 / 0.03 / 0.4 \\
84 & 36591 & 1.50 & 8.33 ± 0.08 & 7.75 ± 0.09 & 8.75 ± 0.11 & 27 & 4.12 & 4.16 ± 0.09 & 14 & 1,4,5 & 11.2$^{+2.2}_{-1.6}$ & 5.2$^{+5.9}_{-3.1}$ & 25$^{+25}_{-25}$ & 0.57 / 0.88 / 0.84 /\textcolor{red}{ 0.16} &  \\
85 & 205021 & 1.50 & 8.24 ± 0.06 & 8.11 ± 0.11 & 8.64 ± 0.13 & 27 & 4.05 & 4.38 ± 0.08 & 32 & 1,4,5,17 & 11.7$^{+1.7}_{-1.7}$ & 9.4$^{+2.4}_{-1.7}$ & 35$^{+25}_{-15}$ & 0.19 / 0.80 / 0.74 / \textcolor{red}{ 0.00} & \$\prescript{\mathrm{m}}{(17,18,22,24)}{}\$76 ± 6 \$\prescript{\mathrm{b}}{(46)}{}\$SB1 / 11 / 0.52 / 0.6 \\
86 & 46328 & 1.36 & 8.18 ± 0.12 & 8.00 ± 0.17 & 8.59 ± 0.17 & 27.5 ± 1.0 & 3.75 ± 0.15 & 4.58 ± 0.07 & 10 & 1,2 & 16.5$^{+3.4}_{-3.4}$ & 8.1$^{+2.3}_{-1.6}$ & 235$^{+65}_{-45}$ & 0.80 / 0.82 / 0.58 /\textcolor{red}{ 0.33} & \$\prescript{\mathrm{m}}{(18,19,20,21,22,24)}{}\$350 ± 10 \\
\textbf{87} & \textbf{3293-003} & \textbf{ 1.3} & \textbf{7.95 ± 0.22} & \textbf{7.68 ± 0.06} & \textbf{8.75 ± 0.20} & \textbf{22.5 ± 1.0} & \textbf{3.00 ± 0.10} & \textbf{4.81 ± 0.06} & \textbf{84} & \textbf{7,9} & \textbf{15.8$^{+1.1}_{-0.8}$} & \textbf{11.2$^{+0.8}_{-1.1}$} & \textbf{465$^{+35}_{-85}$} & \textbf{0.09 / 0.72 / 0.76 / 0.79} &  \\
\textbf{88} & \textbf{3293-002} & \textbf{ 1.2} & \textbf{8.10 ± 0.22} & \textbf{8.11 ± 0.12} & \textbf{8.67 ± 0.15} & \textbf{24.2 ± 1.0} & \textbf{3.00 ± 0.10} & \textbf{5.22 ± 0.05} & \textbf{90} & \textbf{7,9} & \textbf{23.1$^{+1.3}_{-1.8}$} & \textbf{7.1$^{+0.7}_{-0.5}$} & \textbf{425$^{+65}_{-35}$} & \textbf{0.57 / 0.82 / 0.56 / \textcolor{red}{ 0.29}} &  \\
89 & 35468 & 1.01 & 8.11 ± 0.09 & 7.90 ± 0.16 & 8.16 ± 0.27 & 22.0 ± 1.0 & 3.50 ± 0.20 & 3.90 ± 0.06 & 51 & 1,11 & 11.6$^{+2.5}_{-3.6}$ & 15.7$^{+5.2}_{-5.2}$ & 305$^{+65}_{-55}$ & 0.13 / 0.79 / 0.48 /  0.88 & \$\prescript{\mathrm{m}}{(23)}{}\$N/A \$\prescript{\mathrm{b}}{(4)}{}\$SB2? / --- / --- / --- \\
90 & 51309 & 0.84 & 7.89 ± 0.19 & 7.86 ± 0.34 & 8.25 ± 0.44 & 17.5 ± 1.0 & 2.75 ± 0.15 & 5.01 ± 0.20 & 32 & 1,11 & 24.1$^{+2.3}_{-5.9}$ & 6.5$^{+3.1}_{-1.9}$ & 465$^{+35}_{-35}$ & \textcolor{red}{0.00} / \textcolor{red}{0.04} / \textcolor{red}{0.06} / \textcolor{red}{ 0.47} &  \\ \hline

\end{tabular}}
\tablefoot{Key to references: 
[1] \citet{Proffitt2001}; 
[2] \citet{Morel2006}; 
[3] \citet{Mazmumdar2006}; 
[4] \citet{Nieva2012}; 
[5] \citet{Proffitt2015}; 
[6] \citet{Venn2002}; 
[7] \citet{Proffitt2023}; 
[8] \citet{Simon2010,Nieva2011}; 
[9] \citet{Proffitt2016}; 
[10] \citet{Dupret2004}; 
[11] \citet{Morel2008}; 
[12] \citet{Pamyatnykh2004}; 
[13] \citet{Aerts1996}; 
[14] \citet{Neiner2003}; 
[15] \citet{Aerts2006}; 
[16] \citet{Gies1992}; 
[17] \citet{Henrichs2013};
[18] \citet{Rudy1978};
[19] \citet{Hubrig2006};
[20] \citet{Hubrig2009};
[21] \citet{Bagnulo2015};
[22] \citet{Shultz2018};
[23] \citet{Wade2016};
[24] \citet{Schnerr2008};
[25] \citet{Schnerr2006};
[26] \citet{Bagnulo2012};
[27] \citet{Butkovskaya2007};
[28] \citet{Grunhut2017};
[29] \citet{Vitrichenko2002};
[30] \citet{Levato1987};
[31] \citet{Chini2012};
[32] \citet{Abt1978};
[33] \citet{Southworth2004};
[34] \citet{Leone1999};
[35] \citet{Aerts1998};
[36] \citet{Stickland2000};
[37] \citet{Ebbighausen1960};
[38] \citet{Hernandez1980};
[39] \citet{Stickland1996};
[40] \citet{Lehmann2001};
[41] \citet{Miroshnichenko2001};
[42] \citet{Lloyd1995};
[43] \citet{Burssens2020};
[44] \citet{Libich2006};
[45] \citet{Luyten1936};
[46] \citet{Fitch1969}
\\
The typical 1-$\sigma$ error for $\Teff$ ($\logg$) of 1000$\K$ (0.1$\gunit$) is adopted when not provided.}
\end{table*}

==> tab_tmp.tex <==
\begin{table*}[]
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{cccccccc}
\hline \hline
No & Star & $M_\mathrm{evol} (T_\mathrm{eff}, \log L) \, [M_\odot]$ & $M_\mathrm{evol} (T_\mathrm{eff}, \log g)\, [M_\odot]$ & $M_\mathrm{spec}$ & $M_\mathrm{spec,Danny}$ & $M_\mathrm{specc,Danny}$ & $P (f_c)^\mathrm{product} (T_\mathrm{eff}, \log L, \log g)$ \\ \hline
1 & HD 44743 & 12.9$^{+0.8}_{-0.8}$ & 12.2$^{+3.5}_{-2.5}$ & 10.0$^{+4.1}_{4.1}$ & 10.86 ± 4.17 & 10.88 ± 4.17 & 0.535 \\
2 & HD 37023 & 17.1$^{+1.3}_{-1.3}$ & 16.0$^{+1.8}_{-0.8}$ & 53.0$^{+16.4}_{16.4}$ & 55.52 ± 15.34 & 55.61 ± 15.34 & {\color[HTML]{C9211E} 0.000} \\
3 & HD 34816 & 14.6$^{+1.6}_{-0.7}$ & 15.2$^{+1.3}_{-3.1}$ & 21.3$^{+6.6}_{6.6}$ & 22.35 ± 6.23 & 22.38 ± 6.23 & 0.205 \\
4 & HD 142669 & 7.7$^{+0.7}_{-0.4}$ & 7.3$^{+0.9}_{-0.9}$ & 9.2$^{+3.1}_{3.1}$ & 9.56 ± 2.44 & 9.8 ± 2.45 & 0.544 \\
5 & HD 63578 & 11.5$^{+1.5}_{-1.0}$ & 9.0$^{+1.2}_{-0.7}$ & 38.9$^{+13.0}_{13.0}$ & 41.18 ± 11.69 & 41.44 ± 11.71 & {\color[HTML]{C9211E} 0.001} \\
6 & HD 112092 & 6.9$^{+0.3}_{-0.3}$ & 6.5$^{+0.9}_{-0.5}$ & 9.4$^{+3.2}_{3.2}$ & 9.8 ± 2.46 & 9.84 ± 2.46 & 0.309 \\
7 & HD 212978 & 8.2$^{+0.4}_{-1.0}$ & 7.1$^{+1.4}_{-1.0}$ & 10.1$^{+3.6}_{3.6}$ & 10.65 ± 2.83 & 11.08 ± 2.85 & 0.434 \\
8 & HD 36351 & 8.7$^{+0.4}_{-0.7}$ & 7.6$^{+1.2}_{-0.7}$ & 11.5$^{+3.9}_{3.9}$ & 12.11 ± 3.2 & 12.16 ± 3.21 & 0.318 \\
9 & HD 160762 & 6.4$^{+0.4}_{-0.4}$ & 6.1$^{+0.5}_{-0.8}$ & 6.8$^{+2.5}_{2.5}$ & 7.2 ± 1.88 & 7.2 ± 1.88 & 0.771 \\
\textbf{10} & \textbf{3293-015} & \textbf{12.4$^{+1.7}_{-1.2}$} & \textbf{11.9$^{+2.6}_{-2.6}$} & \textbf{9.9$^{+4.4}_{4.4}$} & \textbf{10.70 ± 4.08} & \textbf{13.12 ± 4.16} & \textbf{0.567} \\
11 & HD 35039 & 8.9$^{+0.3}_{-0.2}$ & 9.0$^{+0.6}_{-0.6}$ & 7.9$^{+1.7}_{1.7}$ & 8.19 ± 1.78 & 8.2 ± 1.78 & 0.545 \\
12 & HD 35299 & 9.3$^{+0.4}_{-0.4}$ & 8.8$^{+0.7}_{-0.7}$ & 10.6$^{+3.4}_{3.4}$ & 11.08 ± 2.87 & 11.08 ± 2.87 & 0.582 \\
13 & BD+56 576 & 12.2$^{+0.9}_{-0.9}$ & 11.3$^{+2.5}_{-2.5}$ & 13.5$^{+4.6}_{4.6}$ & 14.34 ± 4.09 & 14.38 ± 4.09 & 0.663 \\
\textbf{14} & \textbf{3293-023} & \textbf{9.0$^{+0.7}_{-0.4}$} & \textbf{9.4$^{+1.4}_{-1.4}$} & \textbf{6.7$^{+2.1}_{2.1}$} & \textbf{6.99 ± 1.80} & \textbf{7.72 ± 1.78} & \textbf{0.353} \\
15 & HD 121790 & 7.5$^{+0.4}_{-0.4}$ & 7.4$^{+0.9}_{-0.9}$ & 7.6$^{+2.5}_{2.5}$ & 7.95 ± 2 & 8.24 ± 2 & 0.851 \\
16 & HD 36430 & 7.0$^{+0.7}_{-0.4}$ & 6.1$^{+0.5}_{-0.5}$ & 15.3$^{+5.3}_{5.3}$ & 16 ± 4.13 & 16.02 ± 4.13 & {\color[HTML]{C9211E} 0.025} \\
17 & HD 64722 & 10.3$^{+1.0}_{-0.4}$ & 10.2$^{+1.4}_{-1.4}$ & 10.5$^{+3.3}_{3.3}$ & 11.09 ± 2.93 & 11.51 ± 2.94 & 0.855 \\
18 & HD 36959 & 10.4$^{+0.5}_{-0.3}$ & 10.7$^{+0.5}_{-0.5}$ & 9.7$^{+1.9}_{1.9}$ & 10 ± 1.98 & 10 ± 1.98 & 0.478 \\
19 & HD 37744 & 9.0$^{+0.5}_{-0.5}$ & 9.4$^{+0.4}_{-0.4}$ & 6.3$^{+1.6}_{1.6}$ & 6.52 ± 1.68 & 6.54 ± 1.68 & {\color[HTML]{C9211E} 0.129} \\
\textbf{20} & \textbf{3293-038} & \textbf{6.7$^{+0.7}_{-0.5}$} & \textbf{7.0$^{+1.4}_{-1.4}$} & \textbf{4.2$^{+1.8}_{1.8}$} & \textbf{4.49 ± 1.67} & \textbf{5.53 ± 1.68} & \textbf{0.226} \\
21 & HD 37017 & 6.2$^{+0.7}_{-0.5}$ & 5.7$^{+0.5}_{-0.5}$ & 7.3$^{+2.6}_{2.6}$ & 7.61 ± 1.95 & 7.98 ± 1.96 & 0.605 \\
22 & HD 122980 & 7.2$^{+0.4}_{-0.2}$ & 7.0$^{+0.9}_{-0.4}$ & 8.4$^{+1.4}_{1.4}$ & 8.58 ± 1.28 & 8.59 ± 1.28 & 0.340 \\
23 & HD 37209 & 9.5$^{+1.0}_{-0.7}$ & 9.7$^{+1.2}_{-1.7}$ & 9.8$^{+3.1}_{3.1}$ & 10.22 ± 2.66 & 10.28 ± 2.66 & 0.870 \\
24 & HD 111123 & 14.2$^{+0.7}_{-1.7}$ & 13.6$^{+4.3}_{-2.4}$ & 7.2$^{+3.8}_{3.8}$ & 8.24 ± 4.54 & 8.32 ± 4.54 & {\color[HTML]{C9211E} 0.198} \\
25 & HD 36629 & 7.2$^{+0.5}_{-0.5}$ & 7.6$^{+0.7}_{-0.7}$ & 6.9$^{+2.3}_{2.3}$ & 7.16 ± 1.84 & 7.16 ± 1.84 & {\color[HTML]{C9211E} 0.104} \\
26 & HD 37020 & 15.1$^{+0.9}_{-0.9}$ & 15.1$^{+0.9}_{-0.9}$ & 17.6$^{+4.7}_{4.7}$ & 18.38 ± 4.9 & 18.43 ± 4.9 & 0.276 \\
\textbf{27} & \textbf{3293-012} & \textbf{12.5$^{+0.9}_{-0.9}$} & \textbf{11.6$^{+2.5}_{-2.5}$} & \textbf{12.7$^{+3.9}_{3.9}$} & \textbf{13.21 ± 3.41} & \textbf{13.56 ± 3.43} & \textbf{0.787} \\
28 & HD 37356 & 9.9$^{+0.6}_{-1.0}$ & 8.6$^{+0.7}_{-1.7}$ & 18.5$^{+6.3}_{6.3}$ & 19.41 ± 5.24 & 19.43 ± 5.24 & {\color[HTML]{C9211E} 0.058} \\
29 & HD 41753 & 6.4$^{+0.4}_{-1.0}$ & 5.9$^{+0.4}_{-0.4}$ & 8.4$^{+3.2}_{3.2}$ & 8.82 ± 2.38 & 8.89 ± 2.39 & 0.368 \\
30 & HD 109668 & 8.8$^{+0.8}_{-0.5}$ & 7.7$^{+1.4}_{-1.0}$ & 15.6$^{+6.0}_{6.0}$ & 16.59 ± 5.43 & 17.04 ± 5.46 & {\color[HTML]{C9211E} 0.129} \\
31 & HD 29248 & 9.4$^{+0.5}_{-0.7}$ & 9.3$^{+0.6}_{-0.6}$ & 8.8$^{+1.6}_{1.6}$ & 9.05 ± 1.58 & 9.07 ± 1.58 & 0.753 \\
32 & HD 38622 & 6.5$^{+0.4}_{-0.4}$ & 7.4$^{+0.7}_{-1.1}$ & 4.1$^{+1.5}_{1.5}$ & 4.31 ± 1.14 & 4.37 ± 1.14 & {\color[HTML]{C9211E} 0.198} \\
33 & HD 120324 & 9.0$^{+0.5}_{-0.8}$ & 9.8$^{+1.8}_{-1.8}$ & 4.8$^{+1.7}_{1.7}$ & 5.15 ± 1.55 & 5.8 ± 1.59 & {\color[HTML]{C9211E} 0.089} \\
34 & HD 202347 & 9.2$^{+0.7}_{-1.0}$ & 8.8$^{+1.2}_{-0.7}$ & 10.1$^{+3.3}_{3.3}$ & 10.64 ± 2.8 & 10.97 ± 2.81 & 0.702 \\
35 & HD 64740 & 8.8$^{+0.7}_{-0.4}$ & 8.6$^{+0.7}_{-1.2}$ & 10.4$^{+3.3}_{3.3}$ & 10.88 ± 2.77 & 11.31 ± 2.78 & 0.594 \\
36 & HD 68243 & 13.2$^{+0.9}_{-1.3}$ & 10.6$^{+1.7}_{-2.3}$ & 26.0$^{+8.5}_{8.5}$ & 27.29 ± 7.58 & 27.71 ± 7.6 & {\color[HTML]{C9211E} 0.035} \\
37 & HD 45546 & 6.9$^{+1.0}_{-0.4}$ & 7.0$^{+2.0}_{-0.7}$ & 4.5$^{+1.7}_{1.7}$ & 4.73 ± 1.39 & 4.82 ± 1.4 & 0.201 \\
38 & HD 24131 & 11.4$^{+0.5}_{-0.9}$ & 10.8$^{+1.4}_{-1.9}$ & 19.7$^{+6.1}_{6.1}$ & 20.62 ± 5.48 & 20.76 ± 5.48 & {\color[HTML]{C9211E} 0.061} \\
\textbf{39} & \textbf{3293-030} & \textbf{7.1$^{+0.4}_{-0.4}$} & \textbf{7.5$^{+1.1}_{-1.8}$} & \textbf{4.3$^{+1.9}_{1.9}$} & \textbf{4.65 ± 1.77} & \textbf{5.73 ± 1.80} & \textbf{0.237} \\
40 & HD 886 & 9.8$^{+1.0}_{-1.0}$ & 8.8$^{+0.7}_{-1.7}$ & 15.1$^{+5.3}_{5.3}$ & 15.96 ± 4.6 & 15.96 ± 4.6 & {\color[HTML]{C9211E} 0.180} \\
41 & HD 143018 & 11.2$^{+1.3}_{-0.9}$ & 11.8$^{+2.0}_{-1.4}$ & 9.8$^{+3.3}_{3.3}$ & 10.34 ± 3.09 & 10.59 ± 3.1 & 0.426 \\
42 & HD 216916 & 10.0$^{+1.0}_{-1.0}$ & 9.2$^{+1.4}_{-1.4}$ & 11.9$^{+3.9}_{3.9}$ & 12.48 ± 3.28 & 12.48 ± 3.28 & 0.508 \\
43 & HD 121743 & 7.7$^{+0.9}_{-0.4}$ & 7.7$^{+1.5}_{-1.0}$ & 7.5$^{+2.5}_{2.5}$ & 7.89 ± 2.07 & 7.99 ± 2.07 & 0.779 \\
44 & HD 35337 & 9.7$^{+1.0}_{-0.4}$ & 8.9$^{+1.2}_{-1.7}$ & 16.2$^{+5.2}_{5.2}$ & 17.06 ± 4.51 & 17.07 ± 4.51 & {\color[HTML]{C9211E} 0.116} \\
\textbf{45} & \textbf{3293-024} & \textbf{9.0$^{+0.5}_{-0.5}$} & \textbf{8.8$^{+1.5}_{-1.5}$} & \textbf{6.5$^{+2.1}_{2.1}$} & \textbf{6.84 ± 1.72} & \textbf{7.54 ± 1.77} & \textbf{0.342} \\
\textbf{46} & \textbf{3293-019} & \textbf{11.6$^{+0.9}_{-0.9}$} & \textbf{11.4$^{+2.1}_{-2.1}$} & \textbf{9.9$^{+3.0}_{3.0}$} & \textbf{7.95 ± 2.05} & \textbf{8.41 ± 2.06} & \textbf{0.627} \\
\textbf{47} & \textbf{3293-028} & \textbf{8.3$^{+0.4}_{-0.4}$} & \textbf{8.3$^{+1.1}_{-1.8}$} & \textbf{7.1$^{+3.0}_{3.0}$} & \textbf{7.66 ± 2.93} & \textbf{8.72 ± 2.96} & \textbf{0.643} \\
48 & HD 180163 & 8.4$^{+0.4}_{-1.1}$ & 7.4$^{+1.1}_{-1.8}$ & 6.7$^{+2.6}_{2.6}$ & 7.06 ± 1.93 & 7.13 ± 1.94 & {\color[HTML]{C9211E} 0.091} \\
49 & HD 22951 & 14.0$^{+1.7}_{-0.7}$ & 12.2$^{+1.4}_{-1.4}$ & 30.1$^{+9.5}_{9.5}$ & 31.71 ± 8.74 & 31.74 ± 8.74 & {\color[HTML]{C9211E} 0.021} \\
50 & HD 110879 & 7.7$^{+0.4}_{-0.7}$ & 7.3$^{+0.5}_{-0.9}$ & 8.4$^{+2.9}_{2.9}$ & 8.94 ± 2.42 & 9.25 ± 2.43 & 0.662 \\
\textbf{51} & \textbf{3293-031} & \textbf{7.7$^{+0.7}_{-0.4}$} & \textbf{7.7$^{+1.5}_{-1.5}$} & \textbf{6.7$^{+2.8}_{2.8}$} & \textbf{7.30 ± 2.69} & \textbf{8.46 ± 2.70} & \textbf{0.673} \\
52 & HD 188252 & 11.3$^{+0.9}_{-0.9}$ & 10.1$^{+2.3}_{-2.3}$ & 14.6$^{+5.0}_{5.0}$ & 15.36 ± 4.23 & 15.8 ± 4.25 & 0.387 \\
53 & HD 214263 & 7.7$^{+0.4}_{-1.0}$ & 6.9$^{+0.9}_{-0.9}$ & 7.5$^{+2.6}_{2.6}$ & 7.81 ± 2.03 & 7.97 ± 2.03 & 0.811 \\
54 & HD 36960 & 14.2$^{+1.0}_{-1.5}$ & 14.4$^{+1.4}_{-3.2}$ & 14.4$^{+4.4}_{4.4}$ & 15.16 ± 4.15 & 15.19 ± 4.15 & 0.909 \\
55 & HD 36285 & 7.4$^{+0.5}_{-0.5}$ & 7.3$^{+0.9}_{-0.9}$ & 7.3$^{+2.4}_{2.4}$ & 7.64 ± 1.98 & 7.64 ± 1.98 & 0.480 \\
56 & HD 56139 & 9.5$^{+0.4}_{-0.6}$ & 8.3$^{+1.5}_{-1.5}$ & 11.5$^{+4.1}_{4.1}$ & 12.17 ± 3.32 & 12.68 ± 3.34 & 0.465 \\
57 & HD 214993 & 10.9$^{+1.0}_{-1.0}$ & 11.9$^{+2.4}_{-2.4}$ & 5.7$^{+1.9}_{1.9}$ & 6.11 ± 1.77 & 6.23 ± 1.77 & {\color[HTML]{C9211E} 0.062} \\
58 & HD 106490 & 10.2$^{+1.1}_{-1.1}$ & 9.6$^{+0.9}_{-1.5}$ & 11.8$^{+4.4}_{4.4}$ & 12.66 ± 4.26 & 13.4 ± 4.32 & 0.598 \\
59 & HD 184171 & 6.4$^{+0.4}_{-0.4}$ & 6.3$^{+0.5}_{-0.5}$ & 4.9$^{+1.9}_{1.9}$ & 5.16 ± 1.39 & 5.19 ± 1.39 & 0.476 \\
\textbf{60} & \textbf{3293-008} & \textbf{12.9$^{+0.8}_{-0.8}$} & \textbf{14.0$^{+2.4}_{-3.4}$} & \textbf{8.7$^{+2.7}_{2.7}$} & \textbf{9.13 ± 2.39} & \textbf{10.08 ± 2.39} & \textbf{0.227} \\
\textbf{61} & \textbf{3293-004} & \textbf{14.7$^{+1.0}_{-1.0}$} & \textbf{19.9$^{+5.0}_{-4.1}$} & \textbf{5.8$^{+1.8}_{1.8}$} & \textbf{6.12 ± 1.64} & \textbf{6.66 ± 1.66} & {\color[HTML]{C9211E} \textbf{0.004}} \\
62 & HD 160578 & 11.1$^{+0.9}_{-0.9}$ & 10.2$^{+1.0}_{-2.4}$ & 16.5$^{+5.4}_{5.4}$ & 17.37 ± 4.65 & 17.9 ± 4.66 & {\color[HTML]{C9211E} 0.199} \\
\textbf{63} & \textbf{3293-010} & \textbf{12.0$^{+0.9}_{-0.9}$} & \textbf{12.6$^{+2.5}_{-2.5}$} & \textbf{9.3$^{+2.9}_{2.9}$} & \textbf{9.77 ± 2.55} & \textbf{9.84 ± 2.51} & \textbf{0.414} \\
\textbf{64} & \textbf{3293-005} & \textbf{13.8$^{+1.3}_{-0.9}$} & \textbf{18.5$^{+4.5}_{-2.5}$} & \textbf{6.1$^{+2.4}_{2.4}$} & \textbf{6.73 ± 2.66} & \textbf{8.96 ± 2.73} & {\color[HTML]{C9211E} \textbf{0.009}} \\
65 & HD 3360 & 8.1$^{+0.4}_{-0.4}$ & 8.4$^{+1.3}_{-1.8}$ & 5.7$^{+2.0}_{2.0}$ & 5.95 ± 1.61 & 5.96 ± 1.61 & 0.306 \\
66 & HD 16582 & 8.5$^{+0.8}_{-0.5}$ & 8.7$^{+1.4}_{-1.4}$ & 6.3$^{+2.2}_{2.2}$ & 6.61 ± 1.88 & 6.61 ± 1.88 & 0.364 \\
67 & HD 108249 & 11.2$^{+1.3}_{-0.6}$ & 11.1$^{+2.4}_{-1.7}$ & 10.3$^{+3.3}_{3.3}$ & 10.78 ± 2.94 & 12.44 ± 3 & 0.677 \\
68 & HD 143275 & 17.2$^{+2.1}_{-2.1}$ & 14.2$^{+2.2}_{-1.4}$ & 38.6$^{+15.6}_{15.6}$ & 42.05 ± 17.2 & 43.21 ± 17.35 & {\color[HTML]{C9211E} 0.037} \\
69 & HD 214680 & 19.1$^{+1.9}_{-1.9}$ & 18.4$^{+2.2}_{-2.2}$ & 26.1$^{+8.1}_{8.1}$ & 27.62 ± 7.91 & 27.69 ± 7.91 & 0.226 \\
70 & HD 93030 & 15.0$^{+1.4}_{-1.4}$ & 15.5$^{+2.2}_{-2.2}$ & 13.7$^{+4.8}_{4.8}$ & 14.56 ± 4.82 & 14.82 ± 4.84 & 0.463 \\
71 & HD 37042 & 13.6$^{+0.8}_{-1.1}$ & 13.3$^{+0.9}_{-0.9}$ & 14.1$^{+2.9}_{2.9}$ & 14.49 ± 2.9 & 14.51 ± 2.9 & 0.222 \\
72 & HD 37481 & 8.6$^{+0.8}_{-0.6}$ & 8.8$^{+1.2}_{-1.2}$ & 7.8$^{+2.5}_{2.5}$ & 8.18 ± 2.12 & 8.27 ± 2.13 & 0.682 \\
73 & HD 108248 & 14.2$^{+0.6}_{-1.1}$ & 13.3$^{+2.3}_{-2.3}$ & 13.8$^{+4.3}_{4.3}$ & 14.45 ± 4.01 & 14.67 ± 4.02 & 0.864 \\
74 & HD 34078 & 18.2$^{+1.3}_{-1.3}$ & 18.9$^{+2.2}_{-3.1}$ & 15.5$^{+4.5}_{4.5}$ & 16.22 ± 4.35 & 16.24 ± 4.35 & 0.504 \\
75 & HD 36512 & 18.8$^{+1.3}_{-1.9}$ & 18.4$^{+2.2}_{-3.1}$ & 23.6$^{+7.2}_{7.2}$ & 24.85 ± 7.02 & 24.87 ± 7.02 & 0.258 \\
\textbf{76} & \textbf{3293-016} & \textbf{11.8$^{+1.0}_{-1.0}$} & \textbf{11.5$^{+2.4}_{-1.5}$} & \textbf{9.4$^{+2.9}_{2.9}$} & \textbf{9.89 ± 2.57} & \textbf{9.97 ± 2.51} & \textbf{0.450} \\
77 & HD 24760 & 14.3$^{+1.7}_{-0.7}$ & 11.9$^{+1.4}_{-1.4}$ & 36.4$^{+11.4}_{11.4}$ & 38.25 ± 10.38 & 38.89 ± 10.4 & {\color[HTML]{C9211E} 0.007} \\
78 & HD 74575 & 10.9$^{+0.6}_{-0.6}$ & 11.5$^{+0.9}_{-0.7}$ & 8.5$^{+1.6}_{1.6}$ & 8.69 ± 1.58 & 8.69 ± 1.58 & {\color[HTML]{C9211E} 0.134} \\
\textbf{79} & \textbf{3293-007} & \textbf{14.9$^{+1.0}_{-1.0}$} & \textbf{17.4$^{+3.3}_{-3.3}$} & \textbf{8.3$^{+2.6}_{2.6}$} & \textbf{8.62 ± 2.31} & \textbf{8.69 ± 2.32} & {\color[HTML]{C9211E} \textbf{0.047}} \\
80 & HD 50707 & 11.9$^{+1.4}_{-1.0}$ & 14.7$^{+2.4}_{-2.4}$ & 5.2$^{+1.7}_{1.7}$ & 5.52 ± 1.52 & 5.58 ± 1.53 & {\color[HTML]{C9211E} 0.015} \\
81 & HD 52089 & 12.4$^{+1.1}_{-0.8}$ & 13.4$^{+3.5}_{-2.5}$ & 7.4$^{+3.0}_{3.0}$ & 8.07 ± 3.08 & 8.11 ± 3.08 & {\color[HTML]{C9211E} 0.195} \\
\textbf{82} & \textbf{3293-006} & \textbf{14.4$^{+1.5}_{-1.5}$} & \textbf{16.6$^{+4.5}_{-3.5}$} & \textbf{6.9$^{+2.6}_{2.6}$} & \textbf{7.54 ± 2.92} & \textbf{9.99 ± 2.99} & {\color[HTML]{C9211E} \textbf{0.046}} \\
83 & HD 30836 & 10.4$^{+1.0}_{-0.7}$ & 11.3$^{+3.5}_{-1.5}$ & 6.2$^{+2.2}_{2.2}$ & 6.6 ± 2.01 & 6.72 ± 2.02 & {\color[HTML]{C9211E} 0.115} \\
84 & HD 36591 & 12.6$^{+0.7}_{-1.2}$ & 12.5$^{+0.9}_{-2.2}$ & 14.6$^{+5.0}_{5.0}$ & 15.43 ± 4.74 & 15.43 ± 4.74 & 0.566 \\
85 & HD 205021 & 14.1$^{+0.7}_{-1.6}$ & 12.5$^{+1.1}_{-2.5}$ & 20.3$^{+6.6}_{6.6}$ & 21.33 ± 6.18 & 21.37 ± 6.18 & {\color[HTML]{C9211E} 0.195} \\
86 & HD 46328 & 15.3$^{+1.1}_{-1.1}$ & 13.6$^{+3.4}_{-2.4}$ & 15.1$^{+6.2}_{6.2}$ & 16.44 ± 6.55 & 16.44 ± 6.55 & 0.796 \\
\textbf{87} & \textbf{3293-003} & \textbf{16.1$^{+0.8}_{-1.1}$} & \textbf{18.4$^{+3.3}_{-3.3}$} & \textbf{10.1$^{+3.2}_{3.2}$} & \textbf{10.61 ± 2.83} & \textbf{10.86 ± 2.86} & {\color[HTML]{C9211E} \textbf{0.092}} \\
\textbf{88} & \textbf{3293-002} & \textbf{23.2$^{+1.8}_{-1.8}$} & \textbf{21.0$^{+6.7}_{-4.0}$} & \textbf{19.7$^{+6.1}_{6.1}$} & \textbf{20.58 ± 5.56} & \textbf{21.22 ± 5.54} & \textbf{0.572} \\
89 & HD 35468 & 9.6$^{+0.4}_{-1.0}$ & 9.6$^{+2.6}_{-2.6}$ & 4.3$^{+2.2}_{2.2}$ & 4.91 ± 2.55 & 4.99 ± 2.55 & {\color[HTML]{C9211E} 0.131} \\
90 & HD 51309 & 26.5$^{+3.0}_{-2.1}$ & 26.2$^{+2.5}_{-2.5}$ & 24.6$^{+15.1}_{15.1}$ & 29.35 ± 20.11 & 29.54 ± 20.15 & {\color[HTML]{C9211E} 0.004} \\ \hline
\end{tabular}}
\end{table*}
